Learning Formal Specifications from Membership and Preference Queries

Active learning is a well-studied approach to learning formal specifications, such as automata. In this work, we extend active specification learning by proposing a novel framework that strategically requests a combination of membership labels and pair-wise preferences, a popular alternative to membership labels. The combination of pair-wise preferences and membership labels allows for a more flexible approach to active specification learning, which previously relied on membership labels only. We instantiate our framework in two different domains, demonstrating the generality of our approach. Our results suggest that learning from both modalities allows us to robustly and conveniently identify specifications via membership and preferences.

==> experiments.tex <==
We motivate the problem setting by learning task specification for a household robot. In particular, the robot should clean up rooms without disturbing humans or human conversations. 

For a number of rooms, we emit signals whenever the room needs cleaning $c_i$ or urgent cleaning $u_i$. 
We can furthermore detect whether there is one or multiple humans in a room $h_i^1$, $h^+_i$.  
The robot emits a signal $r$ that encodes the room in which the robot is, and a signal $b$ when it is busy cleaning (and thus noisy), or $w$ if it is idling. 

There are some obvious parts of the task specification that can be laid out immediately.  A positive example shows that a robot in a room that needs urgent cleaning should clean the room. 
As a negative example, the system should not be idling if there is a room that need urgent cleaning. 
We remark that positive examples can also be feed in a symbolic format, in terms of a partial specification.

Other rules are less obvious. For example, it is unclear whether we should clean in a room with multiple humans, or whether we should first clean a room in which we currently are or first move to a room that urgently needs cleaning, moving out of a room that needs cleaning. We intend to learn the correct specification from the users by presenting membership queries (showing one trace and ask whether this trace is acceptable) and preference queries (asking two or more traces and ask which is preferred).


Finally, let us remark that some of the benefits of task specifications are helpful in this setting; e.g., for a household with two occupants, it is straightforward how to combine task specifications as task specifications are closed under intersection.
The task specification is also relatively robust against changes ot the environment as the signals are over high-level aspects of the room rather than a state-based signal. 
Finally, arguments regarding the explainability of a Boolean signal such as a task specification mean that there is clearer feedback possible to a user. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

